Escaping the poverty trap: modeling the interplay between economic growth and the ecology of infectious disease

The dynamics of economies and infectious disease are inexorably linked: economic well-being influences health (sanitation, nutrition, treatment capacity, etc.) and health influences economic well-being (labor productivity lost to sickness and disease). Often societies are locked into "poverty traps" of poor health and poor economy. Here, using a simplified coupled disease-economic model with endogenous capital growth we demonstrate the formation of poverty traps, as well as ways to escape them. We suggest two possible mechanisms of escape both motivated by empirical data: one, through an influx of capital (development aid), and another through changing the percentage of GDP spent on healthcare. We find that a large influx of capital is successful in escaping the poverty trap, but increasing health spending alone is not. Our results demonstrate that escape from a poverty trap may be possible, and carry important policy implications in the world-wide distribution of aid and within-country healthcare spending.

==> load_packages.tex <==
% Comment them out for PNAS
%\usepackage{authblk} % for affiliations in the title
%\usepackage{endfloat}


\usepackage{float}

%\usepackage[authoryear,sort&compress,longnamesfirst]{natbib} 
\usepackage[round,numbers,sort&compress]{natbib} % for PNAS


\usepackage[margin=3cm, includefoot]{geometry}
\usepackage{lineno} 
\usepackage{tabularx} % in the preamble

\usepackage{minitoc} % for TOC in chapters


\usepackage{amssymb, amsmath}
\usepackage{graphicx}
\usepackage{amsthm}
\usepackage{verbatim}
\usepackage[caption = false]{subfig}
\usepackage{epstopdf}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}

\usepackage{amsmath,amscd}
\usepackage{paralist} % use lists on the same line, e.g.: two things i) this and ii) that.


\usepackage{tikz}
\usetikzlibrary{shapes,arrows}
\usetikzlibrary{calc}

\usepackage{fancyhdr}
\usepackage{setspace}
\usepackage{url}
%\usepackage{enumitem}
\usepackage{enumerate}



==> new_commands.tex <==
\newcommand{\E}{\mathbb{E}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\Bin}{\operatorname{Bin}}
\newcommand{\Beta}{\operatorname{Beta}}
\newcommand{\Bern}{\operatorname{Bern}}
\newcommand{\Prob}{\mathbb{P}}
\renewcommand\Re{\mathcal{Re}}
\renewcommand\Im{\mathcal{Im}}
\newcommand{\Indicator}[1]{\mathbf{1}\left( #1 \right)}
\newcommand{\transpose}[1]{#1^\top}
\newcommand{\logit}{\operatorname{logit}}

\newcommand{\tabheader}[1]{\textbf{#1}}
\newcommand{\td}[1]{\stackrel{\cdot}{#1}}

\newcommand{\logtwo}{\log_{2}}
\newcommand{\indep}{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\setbox0\hbox{$#1#2$}%
\copy0\kern-\wd0\mkern4mu\box0}} 

\newcommand{\method}{LICORS }

%\newcommand{\vnorm}[1]{\left|\left|#1\right|\right|}
\newcommand{\vnorm}[1]{\lVert #1 \rVert}
\newcommand{\metric}[3]{d_{#1}\left( #2 , #3 \right)}
\newcommand{\dx}[2]{\frac{\mathrm{d} #1}{\mathrm{d} #2}} 
\newcommand{\info}[2]{\mathcal{I}\left( #1 ; #2 \right)} 
\newcommand{\ent}[1]{\mathcal{H}\left( #1 \right)}

\newcommand{\LSC}[2]{\field{\mathcal{C}}{#1}{#2}}
\newcommand{\estLSC}[2]{\field{\widehat{\mathcal{C}}}{#1}{#2}}

\newcommand{\avgLSC}[1]{\overline{\mathcal{C}}{(#1)}} 
\newcommand{\estavgLSC}[1]{\overline{\widehat{\mathcal{C}}}{(#1)}} 

\newcommand{\event}[1]{$\lbrace$ #1 $\rbrace$}
%\newcommand{\keywords}[1] {\textbf{Keywords:} #1}
\newcommand{\SIM}[2]{\operatorname{sim}\left( #1 , #2 \right)} 
\newcommand{\card}[1]{| #1 |}
\newcommand{\rank}[1]{\operatorname{rk}\left(#1 \right)}

\newcommand{\KL}[2]{\mathcal{D}_{KL}\left(#1 \mid \mid #2 \right)} 
\newcommand{\SymKLexp}[2]{\frac{\KL{p}{q} + \KL{q}{p}}{2}} 
\newcommand{\symKL}[2]{\mathcal{J}\left(#1 \mid \mid #2 \right)} 
\newcommand{\resistKL}[2]{\mathcal{R}\left(#1 \mid \mid #2 \right)} 
\newcommand{\expKL}[2]{\operatorname{KL}^{\gamma}\left(#1 \mid \mid #2 \right)} 
\newcommand{\resistKLWritten}[2]{\frac{1}{\KL{#1}{#2}} + \frac{1}{\KL{#2}{#1}}} 



\newcommand{\vecS}[1]{\mathbf{#1}}
\newcommand{\field}[3]{#1\left(\vecS{#2}, #3 \right) }

\newcommand{\loss}[2]{\operatorname{loss} \left( #1, #2 \right)}
\newcommand{\error}[1]{\operatorname{err} \left( #1 \right)}

\newcommand{\PLC}{\bigtriangledown}
\newcommand{\FLC}{\bigtriangleup}
\newcommand{\CS}{\epsilon\left( \ell^{-} \right)}


\newcommand{\bigO}[1]{\ensuremath{\operatorname{\mathcal{O}}\bigl(#1\bigr)}}
\newcommand{\littleO}[1]{\ensuremath{\operatorname{o}\bigl(#1\bigr)}}
\newcommand{\OmegaO}[1]{\ensuremath{\operatorname{\Omega}\bigl(#1\bigr)}}


\newcommand{\question}[1]{\textbf{#1} }
\newcommand{\answer}{\vspace{1cm} 
\begin{center}
\rule{0.6\textwidth}{0.5pt}
\end{center}
}

\newcommand{\D}[2]{\frac{\partial #1}{\partial #2}} 
\newcommand{\DD}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\tp}[1]{{#1}^{\ensuremath{\mathsf{T}}}}  
\newcommand{\innerprod}[1]{\langle #1 \rangle}

\newcommand{\quotes}[2]{
\begin{flushright}
\hfill \textit{#1} \hspace{2cm} \\
\vspace{5pt}
\hfill {\textbf{#2}}
\vspace{0.25cm}
\end{flushright}
}


\setlength{\marginparsep}{0.25cm}
\setlength{\marginparwidth}{1.7 cm}
%\newenvironment{edit}[2][Note]{\dag\marginpar{\tiny{\textbf{#1:} {#2}}}}

\newenvironment{edit}[2][Note]{\dag\marginpar{\tiny{\textbf{#1 \foo:} {#2}}}} % comment out this line if you want to remove comments in margin from the pdf, and uncomment next line
%\newenvironment{edit}[2][Note]{}  % uncomment this line to make the comments in the margin disappear from the pdf
%\newenvironment{edit}[2][]{\begin{comment} #1 #2 \end{comment}}

\newenvironment{myemph}[1]{\emph{#1}}

\newcounter{bar}
\newcommand{\foo}{%
        \stepcounter{bar}%
        \thebar}


% TIKZ macro to generate the future and past light cones

%\newenvironment{plc}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{presentation}[theorem]{Presentation}

